SuperLoc: The Key to Robust LiDAR-Inertial Localization Lies in Predicting Alignment Risks

Map-based LiDAR localization, while widely used in autonomous systems, faces significant challenges in degraded environments due to lacking distinct geometric features. This paper introduces SuperLoc, a robust LiDAR localization package that addresses key limitations in existing methods. SuperLoc features a novel predictive alignment risk assessment technique, enabling early detection and mitigation of potential failures before optimization. This approach significantly improves performance in challenging scenarios such as corridors, tunnels, and caves. Unlike existing degeneracy mitigation algorithms that rely on post-optimization analysis and heuristic thresholds, SuperLoc evaluates the localizability of raw sensor measurements. Experimental results demonstrate significant performance improvements over state-of-the-art methods across various degraded environments. Our approach achieves a 54% increase in accuracy and exhibits the highest robustness. To facilitate further research, we release our implementation along with datasets from eight challenging scenarios

==> __tmp/method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Methodology} % 2.0 Page
\begin{figure*}[tb]
  \centering
  \includegraphics[width=.9\linewidth]{superloc_figs/method.pdf}
  \caption{\textbf{System Overview of Proposed Method.} The major contributions of this work are highlighted with a red square. The pipeline begins with LiDAR and IMU measurements, from which point, plane, and line features are extracted. Point-plane correspondences are used for PCA to determine principal and normal directions, which are then analyzed for observability. Confidence values for each state direction are used to generate an observability scan, enabling the incorporation of pose priors into the sensor fusion system to prevent degeneracy. }
  \label{fig:method}
\end{figure*}

% \basti{it would be really nice to show a clear mathematical difference between the existing approach and your proposed methods and what it means in terms of the optimization. As a reviewer it is very confusing since some parts look like traditional optimization and some parts look like a ``hack.'' Even if it is a hack it is clearly useful so putting it in context is important.}
\subsection{System Overview}
The overview of our system is shown in  Fig.~\ref{fig:method}.
The pipeline begins with measurements from LiDAR and IMU. From these inputs, we extract point, plane, and line features. The point-plane correspondence is then used to compute the Principal Component Analysis (PCA), which helps identify the principal and normal directions of the correspondences. These directions are analyzed to estimate observability and obtain confidence values for each state direction. Based on this confidence, we generate an observability scan and actively incorporate pose priors into the sensor fusion system to mitigate degeneracy. The joint optimization process involves multi-metric ICP factor\cite{zhao2021super}, pose priors, and IMU pre-integration\cite{Forster_2015}. Here we mainly explain the predicted alignment risk, observability estimation, and active sensor fusion module. For other modules, readers can refer to \cite{zhao2021super} for the detailed structure and implementation.

\subsection{Predicting Alignment Risk}
Detecting alignment risk before odometry failure is crucial for ensuring high accuracy and robustness, especially under extremely challenging environments. 
% Our system calculates real-time confidence values, ranging from 0 to 1, for both translational and rotational directions based on comprehensive observability analysis. Low confidence in any particular direction indicates localization failure is imminent for that specific degree of freedom. This analysis enables timely prediction of potential failures, as illustrated in  Fig.~\ref{fig:first_figure}.  
Here, we explain how to quantify the alignment risk when registering two point clouds $P$ and $Q$ using point-plane correspondences. We employ a KD-tree to identify $k$ point-pairs $(\mathbf{p}_i, \mathbf{q}_i)$, where each $\mathbf{q}_i$ has an associated normal vector $\mathbf{n}_i$. 
Our objective is to find a rigid-body transformation, comprising a rotation $R$ and a translation $t$, that minimizes the sum of squared distances from each $\mathbf{p}_i$ to the plane tangent to $Q$ at $\mathbf{q}_i$. The alignment error is expressed as:\begin{align}
E &= \sum_{i=1}^{k} \left( (R \mathbf{p}_i + t - \mathbf{q}_i) \cdot \mathbf{n}_i \right)^2\\
%\end{equation}
%we expand and minimize above equation:
%\begin{equation}
&= \sum_{i=1}^{k} \left( \left( (\mathbf{p}_i - \mathbf{q}_i) \cdot \mathbf{n}_i \right) + \mathbf{r} \cdot (\mathbf{p}_i \times \mathbf{n}_i) + \mathbf{t} \cdot \mathbf{n}_i \right)^2 
\label{eq:icp}
\end{align}

Then, the point-plane distance transformed by the vector $[\Delta\mathbf{r}^T \quad \Delta\mathbf{t}^T]$ can be rewrite into:
\begin{equation}
\Delta d_i = 
\begin{bmatrix}
\Delta \mathbf{r}^T & \Delta \mathbf{t}^T
\end{bmatrix}
\begin{bmatrix}
\mathbf{p}_i \times \mathbf{n}_i \\
\mathbf{n}_i
\end{bmatrix}
\label{eq:icp2}
\end{equation}
which reveals that points where $\mathbf{n}_i$ is perpendicular to $\Delta\mathbf{t}$, or $\mathbf{p}_i \times \mathbf{n}_i$ is perpendicular to $\Delta\mathbf{r}$, do not contribute to the error $E$. This insight allows us to directly assess whether the current motion, represented by $[\Delta \mathbf{r}^T \quad \Delta \mathbf{t}^T]$, is constrained by analyzing the orthogonality between these vectors.

For each scan, we can evaluate the rotational and translational stability of correspondences individually to determine if they are constrained by the current motion. This analysis yields the matrix $C$ to assess alignment quality:

\begin{equation}
C  =
\begin{bmatrix}
\mathbf{p}_1 \times \mathbf{n}_1 & \cdots & \mathbf{p}_k \times \mathbf{n}_k \\
\mathbf{n}_1 & \cdots & \mathbf{n}_k
\end{bmatrix}
\begin{bmatrix}
(\mathbf{p}_1 \times \mathbf{n}_1)^T & \mathbf{n}_1^T \\
\vdots & \vdots \\
(\mathbf{p}_k \times \mathbf{n}_k)^T & \mathbf{n}_k^T
\end{bmatrix}
\label{eq:alignment_matrix}
\end{equation}

This formulation enables a precise analysis of how small perturbations in the sensor's position and orientation affect the overall alignment risk. Importantly, this process can be performed before optimization begins, predicting potential alignment risks.

\subsection{Observability Estimation}
Although we can predict the potential alignment risks, we still don't know the observability  associated with the current state estimate. We believe observability reflects the stability of constraints and it should be more intuitive and meaningful if we analyze the observability in the world frame instead of the principal frame of PCA or vehicle frame like other methods\cite{zhang2016degeneracy}. Therefore, based on \eqref{eq:icp2}, we compute  6 values for each correspondence  $\mathbf{p}_i$ in the source cloud $P$ and project it to world frame corresponding to $[\mathbf{X}_w,\mathbf{Y}_w,\mathbf{Z}_w, \mathbf{roll}_w,\mathbf{pitch}_w, \mathbf{yaw}_w]$.
\begin{equation}
\mathbf{Obs}_i = a^2_{2D}(\mathbf{p}_i)
\begin{bmatrix}
|\mathbf{C}_i \cdot \mathbf{X}_w| \\
|\mathbf{C}_i \cdot \mathbf{Y}_w| \\
|\mathbf{C}_i \cdot \mathbf{Z}_w| \\
|\mathbf{n}_i \cdot \mathbf{X}_w| \\
|\mathbf{n}_i \cdot \mathbf{Y}_w| \\
|\mathbf{n}_i \cdot \mathbf{Z}_w|
\end{bmatrix}
\end{equation}
where $\mathbf{Obs}_i$ is the observability analysis of points $\mathbf{p}_i$ in the world coordinates, $\mathbf{C}_i = T_{init}^{w}\mathbf{p}_i \times \mathbf{n}_i$, $T_{init}^{w}$ is the initial guess of scan registration, $ a^2_{2D}(\mathbf{p}_i)$ is a planner scalar defined by $a_{2D}=(\sigma_2-\sigma_3)/\sigma_1$, and $\sigma_i$ are eigenvalues of PCA for normal computation to represent planarity of geometry.

The first three values in $\mathbf{Obs}_i$ indicate the contribution of point $\mathbf{p}_i$ to the observability of sensor rotation (roll, pitch, yaw). The last three values represent its contribution to the observability of sensor translations.
Based on these values, we can assign labels to each correspondence according to which state direction it contributes most. By analyzing the label distribution across all correspondences, we can determine which state directions are less constrained and require assistance from other odometry sources.


We hypothesize that in environments with good structure, observability should be evenly distributed across all state directions. To quantify this, we statistically analyze the number of observability labels, $\mathbf{Obs}_i$, for each scan and normalize the results to a [0-1] range as confidence metric:
\begin{align}
\mathbf{Cov}_{trans} &= 3\left[\frac{N_{\mathbf{Obs}_x} }{N_{\mathbf{Obs}_{sum}} },\frac{N_{\mathbf{Obs}_y} }{N_{\mathbf{Obs}_{sum}} },\frac{N_{\mathbf{Obs}_z} }{N_{\mathbf{Obs}_{sum}} }\right] \\
\mathbf{Cov}_{rot} &= 3\left[\frac{N_{\mathbf{Obs}_{roll}} }{N_{\mathbf{Obs}_{sum}} },\frac{N_{\mathbf{Obs}_{pitch}} }{N_{\mathbf{Obs}_{sum}} },\frac{N_{\mathbf{Obs}_{yaw}} }{N_{\mathbf{Obs}_{sum}} }\right]
\end{align}
These equations provide a normalized measure of observability for translation and rotation of the state and we can easily obtain a 6x6 diagonal covariance matrix $\mathbf{Cov}$.

\subsection{Active Sensor Fusion}
Traditional sensor fusion approaches passively combine all measurements and rely on robust kernel functions to mitigate adverse effects. We propose a more proactive strategy: degeneracy-aware sensor fusion. This actively incorporates additional constraints with proper weighting, particularly in degenerate directions. Our method not only identifies degraded directions but also determines the necessary weight in those directions using the proposed $\mathbf{Cov}$ matrix. 

% \basti{it would be good to make this difference more explicit. Why wouldn't you get the same result from a proper covariance matrix calculation instead of your combination. What would be the mathematical difference?
% }

% \basti{I don't think you say anywhere what $\alpha$ and $\gamma$ actually is. If they are the eigen values then I don't think this is correct since the eigen values really just tell you relative to each other if the problem is observable and you can't really compare them across measurements.}
\subsubsection{Pose Prior Factor}
When degeneracy occurs, we leverage relative poses from alternative odometry sources, denoted as [$\Delta p_j^i$, $\Delta q_j^i$] in local coordinates. These are used to constrain the relative position $\hat \alpha j^i$ and rotation $\hat \gamma j^i$ estimates obtained from joint optimization. We define the covariance matrix for this prior information as $\mathbf{Cov_{prior}}=\mathbf{I_{6x6}}-\mathbf{Cov}$. This approach ensures that constraints are equally distributed across  state directions.
The relative pose factor $\mathbf{e}_{i j}$ is defined:



\begin{equation}
	\mathbf{e}_{i j}^{prior}=\left[ {\begin{array}{*{20}{c}}
{\Delta p_j^i}\\
{\Delta q_j^i}
\end{array}} \right] \ominus \left[ {\begin{array}{*{20}{c}}
{\hat \alpha _j^i}\\
{\hat \gamma _j^i}
\end{array}} \right]
\end{equation}
Notably, in environments with well-distributed constraints, the pose prior carries minimal weight.
\subsubsection{Joint Optimization}

We employ a factor graph approach to minimize all residual terms:

\begin{equation}
\mathop {\min }\limits_{{\mathbf{T}_{i + 1}}} \left\{ {\left. {\begin{array}{*{20}{c}}
{\sum\limits_{p \in {\mathbb{F}_{i}}} {{{\left\| {e_i^{po \to po,li,pl}} \right\|}_{\mathbf{cov}}^2} + } }\\
{\sum\limits_{\left( {i,i + 1} \right) \in \mathcal{B} } {{{\left\| {{e^{imu}}} \right\|}^2} }+\sum\limits_{\left( {i,i + 1} \right) \in \mathcal{B} } {{{\left\| {{e^{prior}}} \right\|}_{\mathbf{cov_{prior}}}^2}}}
\end{array}} \right\}} \right.
\end{equation}

Here, $e^{prior}$ is the relative pose factor, actively fused and weighted by the proposed $\mathbf{Cov_{prior}}$ and $e_i^{po \to po,li,pl}$ represents point-to-point (line, distance) residuals between two keyframes\cite{zhao2021super}, $e^{imu}$ denotes the IMU preintegration factor\cite{Forster_2015}. For more details, please refer to \cite{zhao2021super}.


% \subsection{Active Sensor Fusion}
% When the degeneracy happens, most of the existing solutions passively fuse all the measurements they have and let the robust kernel function to mitigate effects. However, we argue that the sensor fusion process should be degeneracy-aware and actively fuse additional constraints with proper weight, particularly in degenerate directions. In this section, we will illustrate how to achieve active sensor fusion.

% \subsubsection{Pose Prior Factor}
% Based on the previous predicted alignment risk and observability estimation strategy, the proposed method can not only figure out the degraded direction but also inform how much additional weight they need in that direction from the proposed $\mathbf{Cov}$ matrix. Therefore, we can easily add additional relative pose prior on degeneracy direction. Since we hope the observability should be equally distributed and thanks to that our covariance matrix is diagonal, we can set the covariance matrix of pose prior as $\mathbf{Cov_{prior}}=\mathbf{I_{6x6}}-\mathbf{Cov}$. The idea is simple and effective and just let the constraints in all the state direction are equal. In environments with well-distributed constraints, the pose prior carries very low weight.

% We only use relative poses from other source odometry [$\Delta p_j^i$, $\Delta q_j^i$] as local constraints to constrain the estimated relative position $\hat \alpha _j^i$, and rotation $\hat \gamma _j^i$. 
% The relative pose factor $\mathbf{e}_{i j}$ is derived as:

% \begin{equation}
% 	\mathbf{e}_{i j}^{prior}=\left[ {\begin{array}{*{20}{c}}
% {\Delta p_j^i}\\
% {\Delta q_j^i}
% \end{array}} \right] \ominus \left[ {\begin{array}{*{20}{c}}
% {\hat \alpha _j^i}\\
% {\hat \gamma _j^i}
% \end{array}} \right]
% \end{equation}

% \subsubsection{Joint Optimization}
% We then use factor graph \cite{Kaess_2011} to minimize all the residual terms. 

% \begin{equation}
% \mathop {\min }\limits_{{\mathbf{T}_{i + 1}}} \left\{ {\left. {\begin{array}{*{20}{c}}
% {\sum\limits_{p \in {\mathbb{F}_{i}}} {{{\left\| {e_i^{po \to po,li,pl}} \right\|}_{\mathbf{cov}}^2} + } }\\
% {\sum\limits_{\left( {i,i + 1} \right) \in \mathcal{B} } {{{\left\| {{e^{imu}}} \right\|}^2} }+\sum\limits_{\left( {i,i + 1} \right) \in \mathcal{B} } {{{\left\| {{e^{prior}}} \right\|}_{\mathbf{cov_{prior}}}^2}}}
% \end{array}} \right\}} \right.
% \end{equation}

% Where the $e_i^{po \to po,li,pl}$tare point-to-point (line, distance) residuals between two LiDAR keyframes and  $e^{imu}$ is preintegration residual factor and $e^{prior}$ is relative pose factor which is actively added and weighted by proposed $\mathbf{Cov_{prior}}$.


% \begin{equation}
% X^*=\underset{X}{\operatorname{argmin}}\left\{\sum_{i,j \in S}\left\|e_{ij}^{IMU}\right\|^2+\sum_{i,j \in L}\left\|e_{i,j}^{\mathrm{po} \rightarrow {\mathrm{po}, \mathrm{li}, \mathrm{pl}}}\right\|^2\right\}
% \end{equation}



% \subsubsection{Multi-metric ICP Factor}
% To robustly estimate optimal pose estimation, we implement a multi-metric ICP approach \cite{zhao2021super} that jointly minimizes point-to-point, point-to-line, and point-to-plane distance errors. $q$ and $p$ are target and source for each point, line and plane feature. We first use dynamic octree to extract out the correspondence pair for all features \cite{zhao2021super}. The optimal transformation $[R, t]$ can be then obtained by minimizing the following residual terms. 
% \begin{equation}
% \begin{aligned}
% \mathrm{e}_{ij}^{\mathrm{po} \rightarrow \mathrm{po}} &= \mathbf{q}_i-\left(R \mathbf{p}_i+t\right) &\quad& q_i, p_i \in F_{i+1}^{p o} \\ 
% \mathrm{e}_{ij}^{\mathrm{po} \rightarrow \mathrm{li}} &= \mathbf{v}_j \times\left(\mathbf{q}_j-\left(R \mathbf{p}_j+t\right)\right) &\quad& q_j, p_j \in F_{i+1}^{l i} \\ 
% \mathrm{e}_{ij}^{\mathrm{po} \rightarrow \mathrm{pl}} &= \mathbf{n}_k^{\top}\left(\mathbf{q}_k-\left(R \mathbf{p}_k+t\right)\right) &\quad& q_k, p_k \in F_{i+1}^{p l}
% \end{aligned}
% \end{equation}

% where $\mathbf{v}_j$ and  $\mathbf{n}$ are principal and normal vector for features. $\mathrm{e}_i^{\mathrm{po} \rightarrow \mathrm{po}}$, $\mathrm{e}_i^{\mathrm{po} \rightarrow \mathrm{li}}$, and $\mathrm{e}_i^{\mathrm{po} \rightarrow \mathrm{pl}}$ are point-to-point (line, distance) residuals between two LiDAR keyframe i and j. 
% \subsubsection{IMU Preintegration Factor}
% To integrate IMU measurements, we apply the IMU preintegration technique \cite{Forster_2015} to obtain residual terms for our optimization.  The $SO(3)$ matrix $R_{i,j}$ represent rotation information at frame i and j, while $p_{i,j}$ and $v_{i,j}$ denote postion and velocity. The relative motion measurements is computed by taking the differences between these values. The IMU residual $\Delta R_{ij}$, $\Delta{v_{ij}}$, $\Delta{p_{ij}}$ between the frame are calculated using the IMU preintegration kinematic model\cite{Forster_2015}, which incorporates gyroscope and accelerometer measurements. The IMU preintegration $e^{IMU}$ residual factor is then defined as follows,
% \begin{equation}
% e^{IMU}_{ij} = \begin{bmatrix}
% \Delta R_{ij}R_i\left(R_j\right)^{-1} \\
% v_i+R_i * \Delta{v_{ij}}- v_j \\
% p_i+R_i * \Delta{p_{ij}}- p_j
% \end{bmatrix}
% \end{equation}

% \subsubsection{Factor Graph Optimization}
% We then use factor graph \cite{Kaess_2011} to perform a global optimization across residual terms. We use $S$ and $L$ to denote collection of keyframes for IMU and LiDAR. The optimization is solved using Levenberg-Marquardt algorithm.
% \begin{equation}
% X^*=\underset{X}{\operatorname{argmin}}\left\{\sum_{i,j \in S}\left\|e_{ij}^{IMU}\right\|^2+\sum_{i,j \in L}\left\|e_{i,j}^{\mathrm{po} \rightarrow {\mathrm{po}, \mathrm{li}, \mathrm{pl}}}\right\|^2\right\}
% \end{equation}


%%\begin{equation}
%%\begin{aligned}
%&\begin{aligned}
%& R_j=R_i \prod_{k=i}^{j-1} \operatorname{Exp}\left(\left({\boldsymbol{\omega}}_k-\mathbf{b}_k^{gyro}-\boldsymbol{\eta}%_k^{gyro}\right) \Delta t\right) \\
%& v_j=v_i+\mathbf{g} \Delta t_{i j}+\sum_{k=i}^{j-1} \mathrm{R}_k\left({\mathbf{a}}_k-\mathbf{b}_k^{acc}-%\boldsymbol{\eta}_k^{acc}\right) \Delta t \\
%%& p_j=p_i+\sum_{k=i}^{j-1}\left[\mathbf{v}_k \Delta t+\frac{1}{2} \mathbf{g} \Delta t^2+\frac{1}{2} \mathrm{R}%%_k\left({\mathbf{a}}_k-\mathbf{b}_k^{acc}-\boldsymbol{\eta}_k^{acc}\right) \Delta t^2\right]
%%\end{aligned}\\
%%\end{aligned}
%%\end{equation}



% \begin{figure*}[tb]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figs/graph_extreme.pdf}
%   \caption{Proposed factor graph structure. (a) The proposed factor graph consists of tightly coupled scan-to-scan and scan-to-map registration factors along with IMU factors. Old frames that leave the optimization window are marginalized to bound the computation cost. The proposed method enables robust pose estimation in challenging situations including (b) the sensor travels over unmapped places, and (c) point cloud data becomes degenerated. }
%   \label{fig:graph_extreme}
% \end{figure*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Notation}

% Given a map point cloud $\mathcal{M} = \{ {\bm p}_k^M \in \mathbb{R}^3 \mid_{k = 1, \ldots, N^M} \}$, we estimate a time series of sensor states ${\bm x}_t$ in the map frame using measurements of point cloud scans $\mathcal{P}_t = \{ {\bm p}_k^S \in \mathbb{R}^3 \mid_{k = 1, \ldots, N^P} \}$ and IMU data $\mathcal{I}_t = [{\bm a}_t, {\bm \omega}_t]$, where ${\bm a}_t \in \mathbb{R}^3$ and ${\bm \omega}_t \in \mathbb{R}^3$ are the linear acceleration and the angular velocity, respectively. The sensor state to be estimated is defined as:
% \begin{align}
% {\bm x}_t = [ {\bm T}_t, {\bm v}_t, {\bm b}_t ],
% \end{align}
% where ${\bm T}_t = [{\bm R}_t \mid {\bm t}_t] \in SE(3)$ and ${\bm v} \in \mathbb{R}^3$ are respectively the sensor pose and velocity in the map frame, and ${\bm b}_t = [{\bm b}_t^a, {\bm b}_t^\omega] \in \mathbb{R}^6$ is the IMU acceleration and angular velocity bias. Note that we transform scan points into the IMU coordinate frame and consider them as if they are in the same coordinate frame for efficiency and simplicity.

% In the following Sec. \ref{sec:matching_factor} and \ref{sec:imu_factor}, we describe the building blocks of the proposed framework, namely the point cloud registration factor and the preintegrated IMU factor, and then present the proposed factor graph structure in Sec. \ref{sec:factor_graph}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Point Cloud Registration Factor}
% \label{sec:matching_factor}

% To constrain the relative pose between point clouds $\mathcal{P}_i$ and $\mathcal{P}_j$, we use the voxelized GICP (VGICP) registration error factor with GPU acceleration \cite{Koide_2022}. As with GICP \cite{segal2009generalized}, VGICP models each point as a Gaussian distribution ${\bm p}_k \sim \mathcal{N}({\bm \mu}_k, {\bm C}_k)$ representing the local geometrical shape and computes a sum of the distribution-to-distribution distances between corresponding points as follows:
% \begin{align}
% \label{eq:epc}
% e^\text{PC} ( \mathcal{P}_i, \mathcal{P}_j, {\bm T}_i, {\bm T}_j ) &= \sum_{{\bm p}_k \in \mathcal{P}_i} e^\text{D2D} ({\bm p}_k, {\bm T}_i^{-1} {\bm T}_j), \\
% \label{eq:d2d}
% e^\text{D2D}({\bm p}_k, {\bm T}_{ij}) &= {\bm d}_k^\top \left( {\bm C}'_k + {\bm T}_{ij} {\bm C}_k {\bm T}_{ij}^\top \right)^{-1} {\bm d}_k,
% \end{align}
% where ${\bm T}_{ij} = {\bm T}_i^{-1} {\bm T}_j$ is the relative transformation between $\mathcal{P}_i$ and $\mathcal{P}_j$, ${\bm p}'_k \sim \mathcal{N}( {\bm \mu}'_k, {\bm C}'_k)$ is the point in $\mathcal{P}_j$ nearest to ${\bm p}_k$, and ${\bm d}_k = {\bm \mu}'_k - {\bm T}_{ij} {\bm \mu}_k$ is the residual between ${\bm \mu}'_k$ and ${\bm \mu}_k$. The covariance matrix ${\bm C}_k$ is computed from neighboring points of ${\bm p}_k$. To avoid a costly nearest neighbor search, VGICP voxelizes the target point cloud $\mathcal{P}_j$ at a specific resolution $r$ and stores the average of means and covariance matrices of points in each voxel. During cost evaluation, it looks up a voxel corresponding to each input point and computes Eq. \ref{eq:d2d} using the voxel as ${\bm p}'_k$.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Preintegrated IMU Factor}
% \label{sec:imu_factor}

% To efficiently incorporate IMU measurements into the factor graph, we use the preintegration technique \cite{Forster_2015}. Given an IMU measurement (${\bm a}_t$ and ${\bm \omega}_t$), the sensor states evolves over time as follows:
% \begin{align}
% \label{eq:imu_evol_R}
% {\bm R}_{t + \Delta t} &= {\bm R}_t \exp \left( \left( {\bm \omega}_t - {\bm b}_t^{\omega} - {\bm \eta}_k^{\omega} \right) \Delta t \right), \\
% \label{eq:imu_evol_v}
% {\bm v}_{t + \Delta t} &= {\bm v}_t + {\bm g} \Delta t + {\bm R}_t \left( {\bm a}_t - {\bm b}_t^a - {\bm \eta}_t^a \right) \Delta t, \\
% \label{eq:imu_evol_p}
% {\bm t}_{t + \Delta t} &= {\bm t}_t + {\bm v}_t \Delta t + \frac{1}{2} {\bm g} \Delta t^2 + \frac{1}{2} {\bm R}_t \left( {\bm a}_t - {\bm b}_t^a - {\bm \eta}_t^a \right) \Delta t^2,
% \end{align}
% where ${\bm g}$ is the gravity vector and ${\bm \eta}_t^a$ and ${\bm \eta}_t^{\omega}$ represent white noise in the IMU measurement.

% The IMU preintegration factor integrates Eqs. \ref{eq:imu_evol_R} -- \ref{eq:imu_evol_p} between times $i$ and $j$ to obtain the relative sensor motion $\Delta {\bm R}_{ij}$, $\Delta {\bm t}_{ij}$, and $\Delta {\bm v}_{ij}$ \cite{Forster_2015}. Then, the IMU prediction error is calculated as follows:
% \begin{align}
% \begin{split}
% \label{eq:preint_R}
% e^{\text{\it IMU}} ( {\bm x}_i, {\bm x}_j ) &= \| \log \left( \Delta {\bm R}_{ij}^\top {\bm R}_i^\top {\bm R}_j \right) \|^2 \\
% + & \| \Delta {\bm t}_{ij} - {\bm R}_i^\top \left( {\bm t}_j - {\bm t}_i - {\bm v} \Delta t_{ij} - \frac{1}{2} {\bm g} \Delta t_{ij}^2 \right) \|^2 \\
% + & \| \Delta {\bm v}_{ij} - {\bm R}_i^\top \left( {\bm v}_j - {\bm v}_i -{\bm g} \Delta t_{ij} \right) \|^2 .
% \end{split}
% \end{align}
% Because IMU measurements provide a constant amount of sensor motion information independent of the environment structure, they help keep the factor graph well-constrained in environments where point cloud registration factors can be degenerate (e.g., tunnels and long corridors).


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Factor Graph Structure}
% \label{sec:factor_graph}

% Fig. \ref{fig:graph_extreme} (a) illustrates the proposed factor graph structure, which consists of four major elements: scan-to-scan registration factors, scan-to-map registration factors, IMU factors, and marginal factors.

% {\bf Ego-motion estimation:} To estimate the sensor ego-motion, scan-to-scan registration factors are created between scan point clouds. To make the estimation robust to quick sensor motion, we create scan-to-scan registration factors between the latest frame and $N^\text{pre}$ preceding frames (e.g., 3 frames), which results in a densely connected factor graph. IMU factors are created between consecutive frames to help predict the sensor pose and keep the factor graph well-constrained under point cloud degeneration.

% {\bf Map-based drift correction:} To suppress estimation drift, we create scan-to-map registration factors between every frame and the map point cloud. We treat the map point cloud as a static frame and create unary registration factors that constrain only the frame poses. The key idea here is to use the same error function for scan-to-scan and scan-to-map registration factors and jointly minimize them. This structure makes it possible to maintain sensor pose tracking on map boundaries and even in unmapped regions. As shown in Fig. \ref{fig:graph_extreme} (b), even if a frame has only partial overlap with the map and the scan-to-map registration factor becomes degenerate, the latest frame is still well-constrained by the scan-to-scan registration factors, and we can safely incorporate the degenerate scan-to-map registration errors into the factor graph. Furthermore, when there is absolutely no overlap with the map, the factor graph simply falls back to a range inertial odometry estimation and maintains sensor pose tracking. Once the sensor comes back to the map, scan-to-map registration errors are re-activated and smoothly correct the estimation drift while retaining the consecutive frame matching consistency. The proposed graph structure also makes the estimation robust to degeneration of point cloud data. As in Fig. \ref{fig:graph_extreme} (c), the tightly coupled scan-to-map registration factors enable deficient relative pose constraints (5-DoF with ambiguity in the corridor direction in the shown case) to be incorporated into the factor graph to reduce estimation errors.

% {\bf Optimization:} To bound the computation cost, we marginalize old frames that leave the optimization window (e.g., 5 s) and add constant linear factors to compensate for the marginalized factors at the last evaluation point. For factor graph optimization and marginalization, we use the iSAM2 optimizer \cite{Kaess_2011} and its efficient Bayes tree elimination implemented in GTSAM \cite{gtsam}.

% In summary, the objective function of the proposed framework is defined as follows:
% \begin{align}
% \begin{split}
% e(\mathcal{X}) 
% & = \sum_{{\bm x}_i \in \mathcal{X}} \sum_{j=i - N^\text{pre}}^{i - 1} e^\text{PC} ( \mathcal{P}_i, \mathcal{P}_j, {\bm T}_i, {\bm T}_j ) \\
% & + \sum_{{\bm x}_i \in \mathcal{X}} e^\text{PC} ( \mathcal{P}_i, \mathcal{M}, {\bm T}_i, {\bm I}^{6 \times 6} ) \\
% & + \sum_{{\bm x}_i \in \mathcal{X}} e^\text{IMU} ( {\bm x}_{i - 1}, {\bm x}_i ) + \mathcal{C},
% \end{split}
% \end{align}
% where $\mathcal{X}$ is a set of sensor states in the optimization window and $\mathcal{C}$ is a set of linear factors for marginalization.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Gravity Direction Estimation}

% In practice, the gravity direction is useful information that allows aligning the upward directions of scan and map point clouds and enables the search space to be narrowed down for global localization in 4-DoF \cite{Lim_2022} or 3-DoF with an additional sensor height assumption \cite{Kim_2018}. Although the gravity direction can easily be obtained using linear acceleration data when the sensor is stationary, the estimated gravity direction can be affected by sensor motion.

% To aid global localization used for initial pose estimation, we developed a simple and robust gravity direction and IMU state estimation method based on batch optimization. We first estimate the sensor trajectory using only point cloud data. To this end, we use a combination of the continuous time ICP (CT-ICP) \cite{Dellenbach2022} and the voxel-based points container structure (linear iVox) \cite{Bai2022}. Given the estimated sensor trajectory and IMU measurements in a certain optimization window (e.g., 2 s), we create a factor graph that consists of relative pose factors based on the estimated trajectory and preintegrated IMU factors between consecutive frames. The objective function is defined as follows:
% \begin{align}
% \label{eq:init}
% e^\text{Init} (\mathcal{X}) &= \sum_{ {\bm x}_i \in \mathcal{X} } \left( e^\text{RP} ( {\bm x}_{i - 1}, {\bm x}_i ) + e^\text{IMU} ({\bm x}_{i - 1}, {\bm x}_i) \right),
% \end{align}
% where $e^\text{RP} ({\bm x}_i, {\bm x}_j) = \| \log ( \widetilde{\bm T}_{ij}^{-1} {\bm T}_i^{-1} {\bm T}_j ) \|^2$ is the relative pose constraint based on the relative pose measurement $\widetilde{\bm T}_{ij}$ computed from the estimated sensor trajectory. Because this objective function has ambiguity in the translation and yaw-axis rotation, we add a large constant to the diagonal elements of the information matrix of the first pose to fix the gauge freedom and maintain system positive definiteness. As an initial estimate of the very first frame, we compute the average linear acceleration vector and rotate the first frame such that the average linear acceleration vector is aligned with the world gravity direction. The initial rotation of the first frame is given by
% \begin{align}
% {\bm \psi} &= {\bm \mu}^a \times {\bm g}^w, \\
% {\bm R}_0 &= \mathbb{I}^{6 \times 6} + \widehat{{\bm \psi}} + \widehat{\bm \psi}^2 \frac{ (1 - {\bm \mu}^a \cdot {\bm g}^w) }{ | {\bm \psi} | ^ 2 },
% \end{align}
% where ${\bm \mu}^a$ is the normalized average linear acceleration vector, ${\bm g}^w = [0, 0, 1]^T$ is the gravity direction in the world frame, and $\widehat{\cdot}$ is the hat operator to compute the skew symmetric matrix. We use the Levenberg-Marquardt optimizer to minimize Eq. \ref{eq:init}. After optimization, we use the optimized sensor pose, velocity, and IMU bias of the last frame as the initial state of the localization system.

% To demonstrate the usefulness of the gravity direction information for automatic system initialization, we implemented a 2D occupancy gridmap-based global localization algorithm using branch-and-bound search \cite{Hess_2016} \footnote{The implementation of the 2D global localization is available at: \url{https://github.com/koide3/hdl_global_localization}}. In outdoor experiments shown in Sec. \ref{sec:outdoor}, we obtain a 2D slice of scan point clouds using the estimated gravity direction and feed it to the global localization algorithm to obtain an initial position estimate. We then initialize the proposed localization framework with the estimated initial position. Note that we designed the framework so that it can dynamically load a global localization module from a shared library. The framework is agnostic to the global localization algorithm and any 3- or 4-DoF global localization algorithm (e.g., \cite{Lim_2022}) can easily be incorporated into the proposed framework.
